ViCo: Word Embeddings from Visual Co-occurrences

We propose to learn word embeddings from visual co-occurrences. Two words co-occur visually if both words apply to the same image or image region. Specifically, we extract four types of visual co-occurrences between object and attribute words from large-scale, textually-annotated visual databases like VisualGenome and ImageNet. We then train a multi-task log-bilinear model that compactly encodes word "meanings" represented by each co-occurrence type into a single visual word-vector. Through unsupervised clustering, supervised partitioning, and a zero-shot-like generalization analysis we show that our word embeddings complement text-only embeddings like GloVe by better representing similarities and differences between visual concepts that are difficult to obtain from text corpora alone. We further evaluate our embeddings on five downstream applications, four of which are vision-language tasks. Augmenting GloVe with our embeddings yields gains on all tasks. We also find that random embeddings perform comparably to learned embeddings on all supervised vision-language tasks, contrary to conventional wisdom.

==> figures/analysis.tex <==
\begin{figure*}[t]
\vspace{-0.75em}
\begin{center}
\hspace{-2em}\includegraphics[width=0.9\linewidth]{images/analysis.pdf}
\end{center}
\vspace{-0.75em}
\caption{\textbf{Unsupervised and Supervised Analysis.} (a,b) \textbf{Qualitative clustering evaluation with t-SNE:} plots show that ViCo augmented GloVe results in tighter, more homogenous clusters than GloVe. Marker shape encodes the annotated coarse category and color denotes if the word is used more frequently as an {\color{brickred} object} or an {\color{darkblue} attribute}; (c,d) \textbf{Quantitative clustering evaluation:} Plots show clustering performance of different embeddings measured through V-Measure at different number of clusters. All ViCo based embeddings outperform GloVe for both fine and coarse annotations. (Sec.~\ref{sec:unsupervised}); (e,f) \textbf{Partitioning evaluation:} Plots compare the ability of Decision Trees to tease apart (or partition) words into fine or coarse categories at different learning capacities (maximum tree depth). Performance is measured through Accuracy. For fine categories, all ViCo based embeddings except those using \emph{ViCo(linear,200)} are more easily partitioned than GloVe. Coarse categories are quite well represented in GloVe and see smaller improvements due to ViCo relative to fine categories. Random vectors perform poorly in all plots (c-f). (Sec.~\ref{sec:supervised}). See Tab.~\ref{tab:analysis_variants} and Tab.~\ref{tab:analysis_baselines} for performance on other metrics for these tasks which follow a similar trend.}
%\caption{\textbf{Supervised Partitioning Analysis.} The plots compare the ease with which a supervised learning algorithm, such as a Decision Tree can tease apart (or partition) words into fine and coarse level categories in the embedding space at different learning capacities (maximum tree depth). In comparison to GloVe and random embeddings, fine categories are more easily partitioned with ViCo based embeddings except for \emph{GloVe+ViCo(linear,200)}. Coarse categories are already well represented in GloVe with ViCo providing a further boost, especially at lower depths. See Tab.~\ref{tab:analysis_baselines} and Tab.~\ref{tab:analysis_variants} for V-Measure and ARI metrics which follow similar trends. (Sec.~\ref{sec:supervised})}
\label{fig:analysis}
\vspace{-1em}
\end{figure*}

%At the fine level, all embeddings using \emph{ViCo} outperform \emph{GloVe} on all metrics. Coarse categories are quite well represented with \emph{GloVe}, however at higher capacities \emph{GloVe+ViCo(linear)} still outperforms \emph{GloVe}. \emph{random} vectors, while being the worst, perform competitively at large depth trees but perform significantly worse than other embeddings for shallower trees. \emph{GloVe+random} yields no gain over \emph{GloVe}. (Sec.~\ref{sec:supervised})}

==> figures/supervised.tex <==
\begin{figure}[t]
\begin{center}
\hspace{-2em}\includegraphics[width=0.7\linewidth]{images/supervised.pdf}
\end{center}
\vspace{-0.5em}
\caption{\textbf{Supervised Partitioning Analysis.} The plots compare the ease with which a supervised learning algorithm, such as a Decision Tree can tease apart (or partition) words into fine and coarse level categories in the embedding space at different learning capacities (maximum tree depth). In comparison to GloVe and random embeddings, fine categories are more easily partitioned with ViCo based embeddings except for \emph{GloVe+ViCo(linear,200)}. Coarse categories are already well represented in GloVe with ViCo providing a further boost, especially at lower depths. See Tab.~\ref{tab:analysis_baselines} and Tab.~\ref{tab:analysis_variants} for V-Measure and ARI metrics which follow similar trends. (Sec.~\ref{sec:supervised})}
\label{fig:supervised}
\end{figure}

%At the fine level, all embeddings using \emph{ViCo} outperform \emph{GloVe} on all metrics. Coarse categories are quite well represented with \emph{GloVe}, however at higher capacities \emph{GloVe+ViCo(linear)} still outperforms \emph{GloVe}. \emph{random} vectors, while being the worst, perform competitively at large depth trees but perform significantly worse than other embeddings for shallower trees. \emph{GloVe+random} yields no gain over \emph{GloVe}. (Sec.~\ref{sec:supervised})}

==> figures/tsne.tex <==
\begin{figure}[t]
\begin{center}
\hspace{-2em}\includegraphics[width=0.7\linewidth]{images/tsne.pdf}
\end{center}
\vspace{-1em}
\caption{\textbf{t-SNE visualization of word embeddings for coarse categories.} Marker shape encodes the annotated coarse category and color denotes if the word is used more frequently as an {\color{brickred} object} or an {\color{darkblue} attribute}. ViCo augmented GloVe results in tighter more homogenous clusters than GloVe.}
\label{fig:tsne}
\end{figure}

==> figures/tsne_unsupervised.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{images/tsne_unsupervised.pdf}
\end{center}
\vspace{-1em}
\caption{\textbf{Unsupervised Clustering Analysis.} \emph{Top:} t-SNE visualization of word embeddings. Marker shape encodes the annotated coarse category and color denotes if the word is used more frequently as an {\color{brickred} object} or an {\color{darkblue} attribute}. \emph{Bottom:} The plots compare the ability of word vectors to naturally group semantically similar visual concepts at both fine and coarse levels using V-Measure. The results all point to ViCo based embeddings clustering words into natural visual categories better than GloVe. ARI follows a similar trend as reported in Tab.~\ref{tab:analysis_variants} and Tab.~\ref{tab:analysis_baselines}. (Sec~\ref{sec:unsupervised})}%At both levels, on both metrics, \emph{GloVe+ViCo} variants outperform \emph{GloVe} alone. \emph{random} and \emph{GloVe+random} perform poorly on both metrics for both category types. (Sec.~\ref{sec:unsupervised})}
\label{fig:tsne_unsupervised}
\end{figure*}

==> figures/unsupervised.tex <==
\begin{figure}[t]
\begin{center}
\vspace{-0.5em}
\hspace{-2em}\includegraphics[width=0.7\linewidth]{images/unsupervised.pdf}
\end{center}
\vspace{-0.5em}
\caption{\textbf{Unsupervised Clustering Analysis.} The plots compare the ability of word vectors to naturally group semantically similar visual concepts at both fine and coarse levels using V-Measure. The results point to ViCo based embeddings clustering words into natural visual categories better than GloVe. ARI follows a similar trend as reported in Tab.~\ref{tab:analysis_variants} and Tab.~\ref{tab:analysis_baselines}. (Sec~\ref{sec:unsupervised})} 
\label{fig:unsupervised}
\end{figure}

==> sections/sup.tex <==
%\input{tables/analysis_vico_variants.tex}

The supplementary material includes: 
\begin{enumerate}
    \itemsep 0.2em
    \item Supervised Partitioning Analysis (Sec.~\ref{sec:supervised})
    \item Performance on all metrics for both unsupervised clustering and supervised partitioning analysis (Tab.~\ref{tab:analysis_baselines})
    \item Words with coarse and fine annotations used for clustering and partitioning analysis (Tab.~\ref{tab:categories}, Sec.~\ref{sec:words_categories}).
    \item Categories used in the zero-shot analysis (Sec.~\ref{sec:words_categories})
    \item Why are random vectors competitive with learned embeddings on vision-language tasks? (Sec.~\ref{sec:random_vectors_good})
\end{enumerate}

\section{Supervised Partitioning Analysis}~\label{sec:supervised}
The partitioning analysis characterizes how well word embeddings represent the differences between words belonging to different semantic categories \emph{while} sharing some representation with words in the same category. This is done by measuring the ability of a supervised learning algorithm to partition words into high-level categories at different learning capacities.  
Specifically, we use a decision tree classifier trained with Gini impurity as the splitting criterion and a minimum of 2 samples per leaf node. We control model capacity through maximum tree depth. We chose decision trees because: (i) they provide a natural way to control model capacity through depth, and (ii) they can hierarchically partition high dimensional spaces based on a label assignment. 

For evaluation, in addition to accuracy, we also compute ARI and V-Measure on the induced clustering (words with the same predicted label belong to the same cluster). Note that we do not have a train-test split here since our goal is to study the separability of concepts in the embedding space rather than generalization. 

Tab.~\ref{tab:analysis_baselines} shows the average performance across tree depth for the 3 metrics. 
Our main conclusions from the partitioning analysis are as follows: %We study generalization directly through a zero-shot-like analysis in the following section.  

%\noindent
\textbf{ViCo outperforms other embeddings.} \emph{ViCo} embeddings alone are partitioned better than other embeddings. \emph{GloVe+ViCo} yields further improvements.

%\noindent
\textbf{Coarse categories well represented in GloVe.} While \emph{GloVe+ViCo} yields significant gains ($11$ to $27\%$ relative gain) over \emph{GloVe} for fine classes, coarse categories are partitioned quite well with \emph{GloVe} alone and using \emph{ViCo} yields relatively small improvements ($3$ to $6\%$ relative gain).

\section{Consistency across tasks and metrics}
Tab.~\ref{tab:analysis_baselines} shows clustering and partitioning performance for multiple metrics -- ARI and V-Measure for clustering, and Accuracy, ARI, and V-Measure for partitioning analysis. Our key conclusions are consistent across both tasks and metrics: (i) \emph{ViCo} clusters words into visual categories better than other embeddings; (ii) Words in the \emph{ViCo} embedding space are easier to partition into visual categories using a supervised learning algorithm; (iii) \emph{GloVe+ViCo} outperforms all embeddings including \emph{GloVe} and \emph{ViCo} individually, showing the complementary nature of information encoded by the two embeddings. 

%\input{figures/supervised.tex}

\section{Words and Categories}~\label{sec:words_categories}
Tab.~\ref{tab:categories} shows the $495$ words used in our clustering and partitioning analysis annotated with $13$ coarse and $65$ fine categories. The words were selected from the list of most frequent words in the VisualGenome~\cite{krishna2017visualgenome} dataset, and were annotated manually with coarse and fine categories. 

For the zero-shot analysis, we use CIFAR-100~\cite{krizhevsky2009cifar}. The $100$ categories are grouped into $20$ super-categories consisting of $5$ categories each. The super-categories are only used for generating the seen/unseen splits as described in the main submission (Sec.4). All categories and super-categories can be found at the original CIFAR-100 website: \href{https://www.cs.toronto.edu/~kriz/cifar.html}{https://www.cs.toronto.edu/~kriz/cifar.html}.

\section{Why are random vectors competitive with learned embeddings?}~\label{sec:random_vectors_good}

Random vectors are surprisingly competitive with learned embeddings (both GloVe and ViCo) on vision-language tasks. Below, we present a hypothesis for this behavior and test the hypothesis on image to caption retrieval task. \\


\noindent
\textbf{Hypothesis:} \textit{Given enough data, vision-language models learn to transform random vectors to get useful intermediate word representations.} \\


\noindent
\textbf{Test:} Fig.~\ref{fig:effect_train_data} shows the performance of random and learned embeddings when trained on different amounts of training data. We see that learned embeddings have a significant advantage over random ones when the model is trained with only $1$-$2\%$ of the available training data but diminishing gains (green line) are observed with more data. 


\begin{figure}[h]~\label{fig:effect_train_data}
   \begin{center}
   \includegraphics[width=\linewidth]{rebuttal/effect_of_training_data.pdf}
   \end{center}
   \vspace{-1em}
   \caption{Comparing random and learned embeddings for Im2Cap model trained with varying amounts of data. We report average recall across 3 runs because of variance observed during training.}
   %\vspace{-1em}
\end{figure}

\noindent
\textbf{Reason for limited improvement of ViCo over Random and GloVe on VQA and Captioning.} Because of the above hypothesis and availability of sufficient training data for tasks like VQA and Image Captioning, gains due to learned embeddings (for both GloVe and ViCo) are relatively small in comparison to random vectors. 

However, we want to emphasize that our clustering, partitioning, and zero-shot analysis, as well as the discriminative attributes task highlight the advantages of learned embeddings over random embeddings, and ViCo over existing word embeddings. Finally, the ability to represent multiple senses of relatedness (Fig.\ 3 in the main submission) also distinguishes ViCo from existing word embeddings.

==> sections/visual_cooccur_bkp.tex <==
% !TEX root = ../main.tex
\section{Visual Co-occurrences}

To learn meaningful word embeddings from visual co-occurrences, %it is crucial to obtain reliable co-occurrence estimates for different types of co-occurrences. 
reliable count estimates are crucial. 
Large-scale dataset like Visual Genome (dense annotated with objects and attributes) and ImageNet (hierarchical label structure) are good starting points for estimating visual co-occurrences. Specifically, we use object and attribute \emph{synset} (synonym set) annotations in VisualGenome to get \emph{Object-Attribute}, \emph{Attribute-Attribute}, and \emph{Context} co-occurrences. ImageNet \emph{synsets} and their ancestors in WordNet are used to compute \emph{Object-Hypernym} co-occurrences.

In particular, word co-occurrence matrices are obtained by first computing \emph{synset} co-occurrences followed by augmentation using \emph{lemma} words associated with synsets in WordNet. We compute \emph{synset} co-occurrences as follows: {\color{blue}I find the following parts unclear?}
\begin{itemize}
    \itemsep 0em
    \item Let $\mathcal{O}$ and $\mathcal{A}$ denote object and attribute synsets annotated for an image region. Pairs in $\mathcal{O}\times\mathcal{A}$ are added to the  \textbf{\emph{Object-Attribute}} co-occurrence matrix for all regions in VisualGenome.
    \item Pairs in $\mathcal{A}\times\mathcal{A}$ are added to the \textbf{\emph{Attribute-Attribute}} co-occurrence matrix for all regions in VisualGenome.
    \item Let $\mathcal{C}$ be the union of all object annotations in an image. Then pairs in $\mathcal{C}\times \mathcal{C}$ are added to the \textbf{\emph{Context}} co-occurrence matrix for all images in VisualGenome
    \item Let $o$ be an object annotated for an image in ImageNet and $\mathcal{H}$ be the ancestors of $o$. Then pairs in $\{o\cup\mathcal{H}\}\times \{o\cup\mathcal{H}\}$ are added to the \textbf{\emph{Object-Hypernym}} co-occurrence matrix for all images in ImageNet.
\end{itemize}

The \emph{synset} co-occurrence matrices are then converted to word co-occurrence matrices by using WordNet. In WordNet, each \emph{synset} is a collection of \emph{lemmas} which share the same meaning. A \emph{lemma} is a word in canonical form that maps to a single meaning. Let $\mathcal{S}_i$ denote the $i^\text{th}$ synset with $\mathcal{W}_i$ as the set of associated \emph{lemma} words. Then for each co-occurrence of \emph{synset} pairs $(\mathcal{S}_i,\mathcal{S}_j)$, all word pairs in $\mathcal{W}_i \times \mathcal{W}_j$ are added to the word co-occurrence matrix. 

%A \emph{lemma} is a word in canonical form that maps to a single meaning). If a canonical word has multiple meanings (polysemy), different \emph{lemmas} are used to represent each sense of the word. For example, \emph{synset} $car.n.01$, denoting a motor vehicle with four wheels, maps to \emph{lemmas} $car.n.01.car$, $car.n.01.automobile$, $car.n.01.motorcar$. \emph{synset} $car.n.02$ denoting a different sense of the word `car', as in a wheeled vehicle adapted to the rails of railroad, however, maps to $car.n.02.car$, $car.n.02.railway\_car$, $car.n.02.railroad\_car$. We replace all occurrences of $car.n.01$ in VisualGenome or ImageNet with words `car', `automobile', and `motorcar' and those of  $car.n.02$ with words `car', `railway', and `railroad'. 

%For example, synset denoting the particular sense of the word `car', as in a motor vehicle with four wheels, maps to lemma words `car',`auto',`automobile',`motorcar' \etc. However, a synset denoting a different sense of the word `car', as in a wheeled vehicle adapted to the rails of railroad, maps to `car' (a different lemma with the same name), `railway car', `railroad car' etc. While in WordNet each sense of the word is identified using a unique number, we simply use the canonical word or name associated with each lemma. Lemma 

{\color{blue}ref to Tab.\ 1 missing?}

\input{tables/stats.tex}
%Most visual datasets with word annotations have limited vocabulary and typically have single category annotation per image region. Datasets used in multi-label attribute classification research have multiple attributes annotated per image but are also restricted to a small label set due to inherent challenges in obtaining \emph{exhaustive} multi-label annotations for a large number of labels (all labels need to be marked present or absent for each image). Attribute annotations are also usually image-level as opposed to region-level.



==> tables/analysis_baselines.tex <==
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\begin{table*}[h]
\centering
\small
%\vspace{-0.75em}
\begin{tabular}{l|c|cc|cc|ccc|ccc}
& & \multicolumn{4}{c|}{\textbf{Unsupervised Clustering}} & \multicolumn{6}{c}{\textbf{Supervised Partitioning}}\\
& & \multicolumn{2}{c|}{Fine} & \multicolumn{2}{c|}{Coarse} & \multicolumn{3}{c|}{Fine} & \multicolumn{3}{c}{Coarse}\\
\textbf{Embeddings} & \textbf{Dim.} & V & ARI & V & ARI & V & ARI & Acc. & V & ARI & Acc.\\
\hline
random(100) & 100 & 0.34 & 0.00 & 0.15 & 0.00 & 0.55 & 0.32 & 0.49 & 0.59 & 0.55 & 0.72\\
%random(300) & 0.34 & 0.00 & 0.15 & 0.00 & 0.54 & 0.32 & 0.49 & 0.59 & 0.55 & 0.72 \\
GloVe & 300 & 0.50 & 0.15 & 0.52 & 0.38 & 0.70 & 0.48 & 0.64 & 0.77 & 0.74 & 0.84\\
GloVe+random(100) & 300+100 & 0.50 & 0.14 &  0.49 & 0.35 & 0.70 & 0.48 & 0.65 & 0.76 & 0.74 & 0.84\\
\hline
vis-w2v-wiki~\cite{kottur2016visw2v}       & 200     & 0.41 & 0.08 & 0.43 & 0.27 & 0.73 & 0.52 & 0.67 & 0.77 & 0.74 & 0.84 \\
vis-w2v-coco~\cite{kottur2016visw2v}       & 200 & 0.45 & 0.08 & 0.4  & 0.22 & 0.72 & 0.46 & 0.66 & 0.72 & 0.67 & 0.81 \\
GloVe+vis-w2v-wiki & 300+200 & 0.5  & 0.14 & 0.52 & 0.4  & 0.72 & 0.49 & 0.66 & 0.76 & 0.72 & 0.84 \\
GloVe+vis-w2v-coco & 300+200 & 0.52 & 0.16 & 0.55 & \sbest{0.42} & 0.74 & 0.56 & 0.68 & 0.77 & 0.74 & \sbest{0.85} \\
\hline
ViCo(linear,100) & 100 & \sbest{0.60} & \sbest{0.21} & \sbest{0.59} & 0.36 & \sbest{0.76} & \sbest{0.57} & \sbest{0.70} & \sbest{0.78} & \sbest{0.76} & \sbest{0.85}\\
GloVe+ViCo(linear,100) & 300+100 & \best{0.61} & \best{0.23} & \best{0.65} & \best{0.48} & \best{0.78} & \best{0.61} & \best{0.72} & \best{0.81} & \best{0.78} & \best{0.87}\\
%GloVe+ViCo(linear,100, w/o WordNet) & 300+100 & 0.54 & 0.18 & 0.58 & \sbest{0.46} & 0.74 & 0.52 & 0.69 & \sbest{0.80} & \best{0.79} & \best{0.87}\\
\end{tabular}
\vspace{0.5em}
%\caption{\textbf{Comparing ViCo to GloVe, random vectors, and vis-w2v.} All ViCo based embeddings %w or w/o GloVe and w or w/o WordNet outperform GloVe and random vectors. \emph{ViCo(linear,100)} outperforms \emph{vis-w2v}. \emph{GloVe+vis-w2v-*} performs similarly to \emph{GloVe} while \emph{GloVe+ViCo} outperforms both \emph{GloVe} and \emph{ViCo}. Using WordNet yields healthy performance gains but is not the only contributor to performance since \emph{GloVe+ViCo(linear,100, w/o WordNet)} also outperforms \emph{GloVe}. \best{Best} and \sbest{second best} numbers are highlighted in each column.}
\caption{\textbf{Comparing ViCo to other embeddings on clustering and partitioning tasks.} V-Measure for clustering is reported in the main submission. Here we show ARI for clustering, and V-Measure, ARI, and Accuracy for partitioning analysis. Conclusion are consistent across both tasks, and all metrics: (i) \emph{ViCo} alone outperforms \emph{GloVe}, \emph{random}, and \emph{vis-w2v} on all metrics, and their combinations on all but one metric (clustering ARI on coarse categories where \emph{GloVe} and \emph{GloVe+vis-w2v-*} do better); (ii) \emph{GloVe+ViCo} outperforms all other embeddings including \emph{ViCo} and \emph{GloVe}, showing that \emph{ViCo} and \emph{GloVe} encode complementary information.}
\vspace{-1em}
\label{tab:analysis_baselines}
\end{table*}
\renewcommand{\arraystretch}{1}
%\emph{GloVe+ViCo(linear,100)} performs better than both \emph{GloVe} and \emph{ViCo(linear,100)} suggesting that ViCo and GloVe contain useful but complementary information. 

==> tables/analysis_unsup_baselines_w_ari.tex <==
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3pt}
\begin{table}[t]
\centering
\footnotesize
\vspace{-0.75em}
\begin{tabular}{l|c|cc|cc}
%& & \multicolumn{4}{c|}{\textbf{Unsupervised Clustering}} \\
& & \multicolumn{2}{c|}{\textbf{Fine}} & \multicolumn{2}{c}{\textbf{Coarse}}\\
\textbf{Embeddings} & \textbf{Dim.} & V & ARI & V & ARI\\
\hline
random(100) & 100 & 0.34 & 0.00 & 0.15 & 0.00 \\
%random(300) & 0.34 & 0.00 & 0.15 & 0.00 & 0.54 & 0.32 & 0.49 & 0.59 & 0.55 & 0.72 \\
GloVe & 300 & 0.50 & 0.15 & 0.52 & 0.38 \\
GloVe+random(100) & 300+100 & 0.50 & 0.14 &  0.49 & 0.35 \\
\hline
vis-w2v-wiki~\cite{kottur2016visw2v}       & 200     & 0.41 & 0.08 & 0.43 & 0.27 \\
vis-w2v-coco~\cite{kottur2016visw2v}       & 200 & 0.45 & 0.08 & 0.4  & 0.22 \\
GloVe+vis-w2v-wiki & 300+200 & 0.5  & 0.14 & 0.52 & 0.4  \\
GloVe+vis-w2v-coco & 300+200 & 0.52 & 0.16 & 0.55 & 0.42 \\
\hline
ViCo(linear,100) & 100 & \sbest{0.60} & \sbest{0.21} & \sbest{0.59} & 0.36 \\
GloVe+ViCo(linear,100) & 300+100 & \best{0.61} & \best{0.23} & \best{0.65} & \best{0.48} \\
GloVe+ViCo(linear,100, w/o WN) & 300+100 & 0.54 & 0.18 & 0.58 & \sbest{0.46} \\
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Comparing ViCo to other embeddings.} All ViCo based embeddings %w or w/o GloVe and w or w/o WordNet 
outperform GloVe and random vectors. \emph{ViCo(linear,100)} also outperforms \emph{vis-w2v}. \emph{GloVe+vis-w2v} performs similarly to \emph{GloVe} while \emph{GloVe+ViCo} outperforms both \emph{GloVe} and \emph{ViCo}. Using WordNet yields healthy performance gains but is not the only contributor to performance since \emph{GloVe+ViCo(linear,100, w/o WN)} also outperforms \emph{GloVe}. \best{Best} and \sbest{second best} numbers are highlighted in each column.}
\vspace{-1em}
\label{tab:analysis_baselines}
\end{table}
\renewcommand{\arraystretch}{1}
%\emph{GloVe+ViCo(linear,100)} performs better than both \emph{GloVe} and \emph{ViCo(linear,100)} suggesting that ViCo and GloVe contain useful but complementary information. 

==> tables/analysis_unsup_vico_variants_w_ari.tex <==
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\centering
\footnotesize
\vspace{-1em}
\begin{tabular}{l|c|cc|cc}
%& & \multicolumn{4}{c|}{\textbf{Unsupervised Clustering}} \\
& & \multicolumn{2}{c|}{\textbf{Fine}} & \multicolumn{2}{c}{\textbf{Coarse}} \\
\textbf{Embeddings} & \textbf{Dim.} & V & ARI & V & ARI \\
\hline
ViCo(linear,50)    & 50      & 0.57 & 0.19 & 0.56 & 0.35 \\
ViCo(linear,100)   & 100     & \sbest{0.60} & 0.21 & 0.59 & 0.36 \\
ViCo(linear,200)   & 200     & 0.59 & 0.21 & 0.60  & 0.37 \\
ViCo(select,200)   & 200     & 0.59 & 0.2  & 0.60  & 0.38 \\
\hline
GloVe & 300 & 0.50 & 0.15 & 0.52 & 0.38 \\
GloVe+ViCo(linear,50) & 300+50 & 0.60 & 0.21 & \best{0.66} & \best{0.52} \\
GloVe+ViCo(linear,100) & 300+100 & \best{0.61} & \best{0.23} & \sbest{0.65} & 0.48 \\
GloVe+ViCo(linear,200) & 300+200 & \sbest{0.60} & \sbest{0.22} & \sbest{0.65} & \sbest{0.49} \\
GloVe+ViCo(select,200) & 300+200 & 0.57 & 0.21 & 0.63 & 0.48 \\
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Effect of transformations on clustering performance.} The table compares average performance across number of clusters. \emph{linear} variants achieve performance similar to \emph{select} with fewer dimensions. In fact, when used in combination with GloVe, \emph{linear} variants outperform \emph{select}. \best{Best} and \sbest{second best} numbers are highlighted in each column.}
\label{tab:analysis_variants}
\end{table}
\renewcommand{\arraystretch}{1}

==> tables/analysis_vico_variants.tex <==
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\begin{table*}[t]
\centering
\footnotesize
\vspace{-1em}
\begin{tabular}{l|c|cc|cc|ccc|ccc}
& & \multicolumn{4}{c|}{\textbf{Unsupervised Clustering}} & \multicolumn{6}{c}{\textbf{Supervised Partitioning}}\\
& & \multicolumn{2}{c|}{Fine} & \multicolumn{2}{c|}{Coarse} & \multicolumn{3}{c|}{Fine} & \multicolumn{3}{c}{Coarse}\\
\textbf{Embeddings} & \textbf{Dim.} & V & ARI & V & ARI & V & ARI & Acc. & V & ARI & Acc.\\
\hline
ViCo(linear,50)    & 50      & 0.57 & 0.19 & 0.56 & 0.35 & 0.72 & 0.53 & 0.66 & 0.74 & 0.7  & 0.82 \\
ViCo(linear,100)   & 100     & \sbest{0.60} & 0.21 & 0.59 & 0.36 & 0.76 & 0.57 & 0.70 & 0.78 & 0.76 & 0.85 \\
ViCo(linear,200)   & 200     & 0.59 & 0.21 & 0.60  & 0.37 & 0.71 & 0.51 & 0.66 & 0.76 & 0.73 & 0.83 \\
ViCo(select,200)   & 200     & 0.59 & 0.2  & 0.60  & 0.38 & 0.77 & \sbest{0.61} & \best{0.73} & 0.79 & 0.76 & \sbest{0.86} \\
\hline
GloVe & 300 & 0.50 & 0.15 & 0.52 & 0.38 & 0.70 & 0.48 & 0.64 & 0.77 & 0.74 & 0.84\\
GloVe+ViCo(linear,50) & 300+50 & 0.60 & 0.21 & \best{0.66} & \best{0.52} & 0.74 & 0.55 & 0.69 & 0.78 & 0.76 & 0.85 \\
GloVe+ViCo(linear,100) & 300+100 & \best{0.61} & \best{0.23} & \sbest{0.65} & 0.48 & \best{0.78} & \sbest{0.61} & 0.72 & \best{0.81} & \sbest{0.78} & \best{0.87}\\
GloVe+ViCo(linear,200) & 300+200 & \sbest{0.60} & \sbest{0.22} & \sbest{0.65} & \sbest{0.49} & 0.70 & 0.43 & 0.64 & 0.79 & 0.76 & 0.85\\
GloVe+ViCo(select,200) & 300+200 & 0.57 & 0.21 & 0.63 & 0.48 & \best{0.78} & \best{0.63} & \best{0.73} & \sbest{0.80} & \best{0.79} & \sbest{0.86}\\
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Effect of transformations on clustering and partitioning performance.} The table compares average performance across number of clusters (clustering) and tree depth (partitioning). For clustering, \emph{linear} variants perform similarly or better than \emph{select}. For partitioning, too small (50) or large (200) embeddings adversely affect performance. However, at an intermediate embedding size of $100$, \emph{linear} performs competitively with \emph{select} at half the number of dimensions. \best{Best} and \sbest{second best} numbers are highlighted in each column.}
\label{tab:analysis_variants}
\end{table*}
\renewcommand{\arraystretch}{1}

==> tables/categories.tex <==
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{2pt}
\begin{table*}[t]
\centering
\scriptsize
\vspace{-2em}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Coarse Categories} & \textbf{Fine Categories} & \textbf{Words}\\
\hline
food & dessert & muffin, cake, pancake, sweet, candy, dessert, cupcake, 
    doughnut, pastry, sugar\\
    & drinks & coffee, tea, water, juice, beer, wine, alcohol, drink, 
    milk\\
    & fruits & apple, banana, fruit, pineapple, mango, pear, berry, 
    lime, lemon, peach, plum, date\\
    & herbs & oregano, herb, parsley, basil\\
    & meals & lunch, meal, breakfast, dinner\\
    & meats & pepperoni, steak, chicken, meat, pork\\
    & nuts & nut, almond, cashew, pecan, peanut, walnut, hazelnut\\
    & spices & salt,  pepper,  spice,  chili,  garlic,  ginger\\
    & vegetarian & tomato, zucchini, broccoli, vegetable, capsicum, spinach, 
    onion, pea, squash, potato, corn, bean, cabbage, mushroom,
    carrot\\
    & prepared/dishes & dish, chip, tortilla, burger, toast, bagel, pizza, 
    pasta, sauce, salad, bread, pickle, bun, soup, noodle, syrup\\
    & miscellaneous & dough,  cheese,  food,  egg,  wheat,  rice,  butter,  oil\\
\hline
animals & birds & bird, turkey, owl, sparrow, pigeon, ostrich, duck, 
    goose, swan, gull, flamingo, peacock\\
    & farm & ox, cow, goat, cattle, bull, lamb, horse, donkey\\
    & fish & fish, dolphin, shark\\
    & pets & dog, cat, kitten, puppy\\
    & reptiles & snake, reptile, turtle, crocodile, lizard\\
    & wild & zebra, elephant, giraffe, lion, tiger, monkey, antelope, 
    bear, animal, gazelle\\
\hline
colors & colors & red, green, blue, yellow, brown, grey, black, white, 
    orange, purple, pink, cyan, violet, indigo, gold, silver, 
    maroon \\
\hline
appliances & appliances & refrigerator, toaster, oven, burner, dishwasher, 
    blender, microwave, oven, stove, appliance, cooler \\
\hline
electronics & computer & computer, laptop, keyboard, mouse, mousepad, 
    printer\\
    & display & monitor, television, tv, display\\
    & audio & earbud, headphone, speaker, microphone\\
    & communication & cellphone, phone, antenna, radio, telephone\\
    & miscellaneous & electonic, device, digital, clock, camera, 
    electronics\\
\hline
utensils & containers & cup, bowl, utensil, plate, jar, vase, urn\\
    & drinks & glass, bottle, jug\\
    & cutlery & spoon, spatula, fork\\
    & cooking/brewing & pan, kettle, teapot, pot\\
\hline
transport & fourwheel & car, bus, minivan, tractor, buggy, van, 
    minivan, jeep\\
    & twowheel & scooter, bike, bicycle, motorcycle, moped\\
    & rail & train, tram, railway, engine\\
    & water & boat, ship, kayak\\
    & air & aircraft, helicopter, jet, aeroplane, propeller\\
    & generic & vehicle, transport, cargo\\
\hline
humans & profession & worker, firefighter, fireman, doctor, soldier, 
    photographer, accountant, refree, student\\
    & male & man, male, boy, father\\
    & female & female, woman, girl, miss, mother, lady, girl\\
    & neutral & people, person, individual, friend, lodger\\
    & color & caucasian, brunet, blonde\\
    & sport & skier, snowboarderskateboarder\\
    & age & young, old, adolescent, teen, teenager, adult, child, 
    baby\\
    & commute & motorcyclist, cyclist, driver, bicyclist, motorist, 
    pedestrian, rider\\
\hline
numbers & numbers & numeral, number, one, two, three, four, five, six, seven, eight, nine, ten \\
\hline
clothes & arms & wristband, mitten, glove, sleeve, watch\\
    & coats & robe, blazer, jacket, coat\\
    & full body & dress, apparel, suit, outfit, clothing, uniform, 
    overall, full-dress\\
    & head & sunglasses, spectacle, visor, helmet, beanie, cap, hat, 
    headband, bandanna, hood\\
    & legs & boot, sandal, shoe, slipper, legging, trouser, skirt, 
    sock, jean, hosiery, stocking, pajama\\
    & neck & bib, tie, scarf, necktie\\
    & undergarments & swimsuit, bikini, lingerie, negligee\\
    & torso & shirt, tshirt, t-shirt, top, blouse, apron, jersey, 
    sweatshirt, sweater, lapel\\
\hline
construction & indoors & bedroom, room, stairway, hallway, patio, kitchen, 
    bathroom, railing, balcony, ledge, lounge\\
    & outdoors & ledge, balcony, roof, rooftop\\
    & buildings & hotel, hostel, lodge, building, church, barn, 
    shed, restaurant, church, hut\\
    & commercial & booth, stall, market, plaza, shop, shopfront, 
    mall\\
    & fixtures & door, window, knob, faucet, lightbulb, bulb, latch, 
    chandelier, fixture, sink, fireplace, bathtub\\
    & furniture & \makecell{chair, table, countertop, counter, cabinet, desk, bed, 
    bench, cupboard, furniture, bookcase, \\armchair, sofa, bench, pew, 
    stool, armchair, bookcase, seat, couch}\\
\hline 
actions & actions & \makecell{call, take, step, come, get, bit, rid, throw, catch, 
    enjoy, smile, eat, look, walk, stand, kneel, crouch, bend, 
    talk, leave, construct, make, hit, keep, \\play, wait, relax, 
    sit, read, serve, fix, lean, leave, kick, squat, bow, swing, 
    get, go, gravel, annoy, rest, put, sleep, catch} \\
\hline
bodyparts & face & ear, nose, nostril, head, lip, cheek, face, tounge, tooth, chin, thumb, elbow\\
    & hair & hair, feather, tuft, eyebrow, brow, mane, eyelash, fur, ponytail, beard\\
    & limbs & leg, arm, foot, thigh, calf, limb\\
    & joints & knee, wrist, ankle, shoulder\\
    & torso & thorax, waist, stomach, belly, abdomen, neck, hip\\
    & extremeties & fingernail, finger, toe, toenail, hand\\
    & non-human & tail, horn, claw, hoof \\
\hline
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Words and Categories.} $495$ words annotated with $13$ coarse and $65$ fine categories used in our clustering and partitioning analysis. Words were selected based on their frequency in VisualGenome and manually annotated with categories.}
\label{tab:categories}
\vspace{-1em}
\end{table*}
\renewcommand{\arraystretch}{1.0}

==> tables/discr_attr.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[h]
\small
\centering
\begin{tabular}{l|c}
\textbf{Embeddings} & \textbf{F1} \\
\hline
GloVe & $63.85 \pm 0.04$ \\
GloVe + ViCo (select, 200 dim.) & \boldmath$64.40 \pm 0.23$  \\
GloVe + ViCo (linear, 50 dim.) & $63.05 \pm 0.15$ \\
GloVe + ViCo (linear, 100 dim.) & \underline{\boldmath$64.46 \pm 0.17$}
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Capturing Discriminative Attributes.}}
\end{table}


==> tables/embeddings.tex <==
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{2pt}
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{lcccc}~\label{tab:embeddings}
\textbf{Embedding} & \textbf{Dim.} & \textbf{Description} & \textbf{Textual} & \textbf{Visual} \\
\midrule
\emph{random} & 100 & \makecell{Randomly sampled from \\uniform distribution} & \xmark & \xmark \\
\hline
\emph{ViCo(linear)} & 100 & \makecell{ViCo \\ Transform: \emph{Linear (100)}} & \xmark & \cmark \\
\hline
\emph{ViCo(select)} & 200 & \makecell{ViCo \\ Transform: \emph{Select}} & \xmark & \cmark \\
\hline
\emph{GloVe} & 300 & GloVe & \cmark & \xmark \\
\hline
\emph{GloVe+random} & 400 & concat(\emph{GloVe}, \emph{random}) & \cmark & \xmark \\
\hline
\emph{GloVe+ViCo(linear)} & 400 & concat(\emph{GloVe}, \emph{ViCo(linear)}) & \cmark & \cmark \\
\hline
\emph{GloVe+ViCo(select)} & 500 & concat(\emph{GloVe}, \emph{ViCo(select)}) & \cmark & \cmark
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Summary of embeddings analysed.} Last two columns indicate the source of co-occurrence information encoded.}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> tables/refexp.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[h]
\small
%\footnotesize
\centering
\begin{tabular}{l|c|c|c}
\textbf{Embeddings} & \textbf{Val} & \textbf{TestA} & \textbf{TestB} \\
\hline
GloVe & $72.2$ & $75.3$ & $66.8$ \\
GloVe + ViCo (select, 200 dim.) & $72.5$  & \underline{\boldmath$76.0$} & \boldmath$67.2$ \\
GloVe + ViCo (linear, 50 dim.) & \boldmath$72.7$ & \boldmath$75.5$ & \underline{\boldmath$67.5$} \\
GloVe + ViCo (linear, 100 dim.) & \underline{\boldmath$73.0$} & \underline{\boldmath$76.0$} & \boldmath$67.2$
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Referring Expression localization accuracy on RefCOCO+ dataset (UNC split).}}
\end{table}


==> tables/tasks.tex <==
\setlength{\tabcolsep}{2.7pt}
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{l|l|c|cc|cccc|ccc|cccc}
& & \textbf{Discr. Attr.} & \multicolumn{2}{c|}{\textbf{Im-Cap Retrieval}} & \multicolumn{4}{c|}{\textbf{VQA}} & \multicolumn{3}{c|}{\textbf{Ref. Exp.}} & \multicolumn{4}{c}{\textbf{Image Captioning}}\\ 
& & Avg. F1 & \multicolumn{2}{c|}{Recall@1} & \multicolumn{4}{c|}{Accuracy} & \multicolumn{3}{c|}{Loc. Accuracy} & \multicolumn{4}{c}{Captioning Metrics}\\ 
\textbf{Embeddings}            & \textbf{Dim.} & $m\pm \sigma$                   & Im2Cap & Cap2Im & Overall & Y/N & Num. & Other & Val & TestA & TestB & B1 & B4 & C & S \\
\hline
\textbf{random}                & 300           & 50.03 $\pm$ 2.26         & 43.1                   & 30.6            & 66.1             & 82.0            & 44.8            & 57.5           & 71.3                & 73.5           & 66.3           & \sbest{0.714}  & \sbest{0.296}  & \sbest{0.910}  & \sbest{0.170}          \\
\textbf{GloVe}                 & 300           & 63.85 $\pm$ 0.04         & 44.8                   & 33.5            & 67.5             & 83.8            & \sbest{46.5}    & \sbest{58.3}   & 72.2                & 75.3           & 66.8           & 0.708          & 0.290          & 0.891          & 0.167          \\
\textbf{GloVe + random}        & 300+100       & 63.88 $\pm$ 0.03         & 44.3                   & \sbest{34.4}    & 67.5             & 84.1            & 45.9            & 58.2           & 72.5                & 75.1           & \sbest{67.5}   & 0.707          & 0.288          & 0.881          & 0.166          \\
\hline
\textbf{GloVe + ViCo (linear)} & 300+50        & 63.05 $\pm$ 0.15         & \best{47.4}            & 34.2            & \best{67.7}      & \best{84.4}     & 46.4            & \sbest{58.3}   & 72.5                & \best{76.0}    & 67.3           & 0.705          & 0.286          & 0.882          & 0.166          \\
\textbf{GloVe + ViCo (linear)} & 300+100       & \best{64.46 $\pm$ 0.17}  & \sbest{46.3}           & 34.2            & \best{67.7}      & \best{84.4}     & \best{46.6}     & \best{58.4}    & 72.7                & 75.5           & \sbest{67.5}   & 0.711          & 0.291          & 0.894          & 0.168          \\
\textbf{GloVe + ViCo (linear)} & 300+200       & \sbest{64.42 $\pm$ 0.39} & 45.1                   & 34.3            & 66.6             & 82.5            & 45.7            & 57.8           & \best{73.4}         & 74.8           & \best{67.7}    & 0.708          & 0.290          & 0.891          & 0.167          \\
\textbf{GloVe + ViCo (select)} & 300+200       & 64.40 $\pm$ 0.23         & 45.6                   & \best{34.5}     & 66.6             & 82.6            & 46.0            & 57.7           & \sbest{73.0}        & \best{76.0}    & 67.2           & \best{0.723}   & \best{0.303}   & \best{0.934}   & \best{0.174}         
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Performance of Embeddings on Vision-Language tasks.}}
\end{table*}

==> tables/tasks_baslines_bkp.tex <==
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{2.7pt}
\begin{table*}[t]
\footnotesize
\centering
\vspace{-0.75em}
\begin{tabular}{l|l|c|cc|cccc|ccc|cccc}~\label{tab:tasks_baselines}
& & \textbf{\color{brickred}Discr. Attr.} & \multicolumn{2}{c|}{\textbf{\color{darkblue}Im-Cap Retrieval}} & \multicolumn{4}{c|}{\textbf{\color{darkblue}VQA}} & \multicolumn{3}{c|}{\textbf{\color{darkblue}Ref. Exp.}} & \multicolumn{4}{c}{\textbf{\color{darkblue}Image Captioning}}\\ 
& & Avg. F1 & \multicolumn{2}{c|}{Recall@1} & \multicolumn{4}{c|}{Accuracy} & \multicolumn{3}{c|}{Loc. Accuracy} & \multicolumn{4}{c}{Captioning Metrics}\\ 
\textbf{Embeddings}            & \textbf{Dim.} & $m\pm \sigma$                   & Im2Cap & Cap2Im & Overall & Y/N & Num. & Other & Val & TestA & TestB & B1 & B4 & C & S \\
\hline
\textbf{random}                & 300           & 50.03 $\pm$ 2.26         & 43.1                   & 30.6            & 66.1             & 82.0            & 44.8            & 57.5           & 71.3                & 73.5           & 66.3           & \best{0.714}   & \best{0.296}   & \best{0.910}   & \best{0.170}          \\
\textbf{GloVe}                 & 300           & 63.85 $\pm$ 0.04         & 44.8                   & 33.5            & 67.5             & 83.8            & \sbest{46.5}    & \sbest{58.3}   & 72.2                & \sbest{75.3}   & 66.8           & 0.708          & 0.290          & 0.891          & 0.167          \\
\textbf{GloVe + random}        & 300+100       & 63.88 $\pm$ 0.03         & 44.3                   & \sbest{34.4}    & 67.5             & 84.1            & 45.9            & 58.2           & \sbest{72.5}        & 75.1           & \best{67.5}    & 0.707          & 0.288          & 0.881          & 0.166          \\
\textbf{GloVe + ViCo (linear)} & 300+100       & \best{64.46 $\pm$ 0.17}  & \sbest{46.3}           & 34.2            & \best{67.7}      & \best{84.4}     & \best{46.6}     & \best{58.4}    & \best{72.7}         & \best{75.5}    & \best{67.5}    & \sbest{0.711}  & \sbest{0.291}  & \sbest{0.894}  & \sbest{0.168}   \\
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Comparing ViCo to GloVe and random vectors.} \emph{GloVe+ViCo(linear)} outperforms \emph{GloVe} and \emph{GloVe+random} for all tasks and outperforms \emph{random} for all tasks except Image Captioning. While random vectors perform close to chance on the \textbf{\color{brickred}word-only} task, they compete tightly with learned embeddings on \textbf{\color{darkblue}{vision-language}} tasks. This suggests that vision-language models are relatively insensitive to choice of word embeddings. \best{Best} and \sbest{second best} numbers in each column are highlighted.}
\vspace{-1em}
\end{table*}
\renewcommand{\arraystretch}{1}

==> tables/tasks_vico_variants.tex <==
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{2.7pt}
\begin{table*}[t]
\footnotesize
\centering
\vspace{-0.75em}
\begin{tabular}{l|l|c|cc|cccc|ccc|cccc}~\label{tab:tasks_variants}
& & \textbf{\color{brickred}Discr. Attr.} & \multicolumn{2}{c|}{\textbf{\color{darkblue}Im-Cap Retrieval}} & \multicolumn{4}{c|}{\textbf{\color{darkblue}VQA}} & \multicolumn{3}{c|}{\textbf{\color{darkblue}Ref. Exp.}} & \multicolumn{4}{c}{\textbf{\color{darkblue}Image Captioning}}\\ 
& & Avg. F1 & \multicolumn{2}{c|}{Recall@1} & \multicolumn{4}{c|}{Accuracy} & \multicolumn{3}{c|}{Loc. Accuracy} & \multicolumn{4}{c}{Captioning Metrics}\\ 
\textbf{Embeddings}            & \textbf{Dim.} & $m\pm \sigma$                   & Im2Cap & Cap2Im & Overall & Y/N & Num. & Other & Val & TestA & TestB & B1 & B4 & C & S \\
\hline
\textbf{GloVe + ViCo (linear)} & 300+50        & 63.05 $\pm$ 0.15         & \best{47.4}            & 34.2            & \best{67.7}      & \best{84.4}     & \sbest{46.4}    & \sbest{58.3}   & 72.5                & \best{76.0}    & 67.3           & 0.705          & 0.286          & 0.882          & 0.166          \\
\textbf{GloVe + ViCo (linear)} & 300+100       & \best{64.46 $\pm$ 0.17}  & \sbest{46.3}           & 34.2            & \best{67.7}      & \best{84.4}     & \best{46.6}     & \best{58.4}    & 72.7                & 75.5           & \sbest{67.5}   & \sbest{0.711}  & \sbest{0.291}  & \sbest{0.894}  & \sbest{0.168}          \\
\textbf{GloVe + ViCo (linear)} & 300+200       & \sbest{64.42 $\pm$ 0.39} & 45.1                   & \sbest{34.3}    & 66.6             & 82.5            & 45.7            & 57.8           & \best{73.4}         & 74.8           & \best{67.7}    & 0.708          & 0.290          & 0.891          & 0.167          \\
\textbf{GloVe + ViCo (select)} & 300+200       & 64.40 $\pm$ 0.23         & 45.6                   & \best{34.5}     & 66.6             & 82.6            & 46.0            & 57.7           & \sbest{73.0}        & \best{76.0}    & 67.2           & \best{0.723}   & \best{0.303}   & \best{0.934}   & \best{0.174}         
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Comparison of ViCo variants on {\color{brickred}word-only} and {\color{darkblue}{vision-language}} tasks.} \emph{GloVe+ViCo(linear,100)} provides the best trade-off between performance and dimensionality. \best{Best} and \sbest{second best} numbers in each column are highlighted.}
\end{table*}
\renewcommand{\arraystretch}{1}

==> tables/vqa.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[h]
\small
%\footnotesize
\centering
\begin{tabular}{l|c|c|c|c}
\textbf{Embeddings} & \textbf{Yes/No} & \textbf{Num.} & \textbf{Other} & \textbf{Overall} \\
\hline
GloVe & $83.8$ & \boldmath$46.5$ & $58.3$ & \boldmath$67.4$ \\
GloVe + ViCo (select, 200 dim.) & $82.6$  & $46.0$ & $57.7$ & $66.6$ \\
GloVe + ViCo (linear, 50 dim.) & \boldmath$84.4$ & $46.4$ & \boldmath$58.3$ & \underline{\boldmath$67.7$}\\
GloVe + ViCo (linear, 100 dim.) & \underline{\boldmath$84.4$} & \underline{\boldmath$46.6$} & \underline{\boldmath$58.4$} & \underline{\boldmath$67.7$}
\end{tabular}
\vspace{0.5em}
\caption{\textbf{VQA v2.0 test-dev accuracies.}}
\end{table}


==> tables/vsepp.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[h]
\small
\centering
\begin{tabular}{l|c|c}
& \multicolumn{2}{c}{\textbf{Recall@1}} \\
\textbf{Embeddings} & \textbf{Im. to Cap.} & \textbf{Cap. to Im.}\\
\hline
GloVe & $44.8$ & $33.5$ \\
GloVe + ViCo (select, 200 dim.) & $45.6$ & \underline{\boldmath$34.5$} \\
GloVe + ViCo (linear, 50 dim.) & \underline{\boldmath$47.4$}  & \boldmath$34.2$\\
GloVe + ViCo (linear, 100 dim.) & \boldmath$46.3$ & \boldmath$34.2$
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Caption-Image Retrieval on MS-COCO.}}
\end{table}

